Crater 2: An Extremely Cold Dark Matter Halo

We present results from MMT/Hectochelle spectroscopy of red giant candidate stars along the line of sight to the recently-discovered Galactic satellite Crater 2. Modelling the joint distribution of stellar positions, velocities and metallicities as a mixture of Crater 2 and Galactic foreground populations, we identify 62 members of Crater 2, for which we resolve line-of-sight velocity dispersion 2.7 +/- 0.3 km/s about mean velocity of 87.5 +/- 0.4 km/s. We also resolve a metallicity dispersion 0.22 about a mean of [Fe/H]=-1.98 +/- 0.1 that is 0.28 +/- 0.14 poorer than is estimated from photometry. Despite Crater 2's relatively large size (projected halflight radius R(h)=1 kpc) and intermediate luminosity (M_V =-8), its velocity dispersion is the coldest that has been resolved for any dwarf galaxy. These properties make Crater 2 the most extreme low-density outlier in dynamical as well as structural scaling relations among the Milky Way's dwarf spheroidals. Even so, under assumptions of dynamical equilibrium and negligible contamination by unresolved binary stars, the observed velocity distribution implies a gravitationally dominant dark matter halo, with dynamical mass 4.4 x 10^6 Msun and mass-to-light ratio M/L=53 enclosed within a radius of 1 kpc, where the equivalent circular velocity is 4.3 km/s.

==> cra2_sspptable1_mnras_all.tex <==
\begin{table*}
\scriptsize
\caption{Hectochelle Stellar Spectroscopy of Crater 2}
\begin{tabular}{@{}ccccccccccccccccccccccc@{}}
\hline
\\
ID&$\alpha_{2000}$&$\delta_{2000}$&$g$&$i$&HJD$^{b}$&S/N$^{c}$&$v_{\rm los}$&$T_{\rm eff}$&$\log_{10}[g/$(cm/s$^{2}$)]&$\mathrm{[Fe/H]}$\\

& [hh:mm:ss]&[$^{\circ}$:$\arcmin$:$\arcsec$]&[mag]&[mag]&[days]&&[km s$^{-1}$]$^{d}$&[K]&[dex]&[dex]\\
\hline
Cra2-001&11:49:34.89&-18:23:27.2&$ 18.95$&$ 17.42$&$  7505.64$&$  8.5$&$  15.3\pm       0.4$&$4869\pm  37$&$5.13\pm0.15$&$-0.12\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-002&11:49:50.39&-18:23:59.5&$ 18.85$&$ 17.44$&$  7505.64$&$  8.5$&$  86.2\pm       0.4$&$4598\pm  81$&$1.09\pm0.14$&$-1.86\pm0.09$\\%$1.000_{-0.000}^{+0.000}$
Cra2-003&11:46:59.26&-18:41:38.0&$ 18.87$&$ 17.45$&$  7505.64$&$  8.6$&$  94.2\pm       0.4$&$4547\pm  83$&$1.44\pm0.20$&$-1.98\pm0.09$\\%$0.999_{-0.001}^{+0.000}$
Cra2-004&11:49:22.24&-18:32:25.9&$ 18.84$&$ 17.46$&$  7505.64$&$  9.8$&$  89.5\pm       0.5$&$4779\pm  82$&$1.21\pm0.20$&$-2.00\pm0.10$\\%$1.000_{-0.000}^{+0.000}$
Cra2-005&11:48:22.55&-17:59:41.2&$ 18.83$&$ 17.41$&$  7505.64$&$ 10.2$&$  88.2\pm       0.5$&$4607\pm  94$&$1.12\pm0.15$&$-2.41\pm0.10$\\%$1.000_{-0.000}^{+0.000}$
Cra2-006&11:47:56.76&-18:04:09.2&$ 18.91$&$ 17.50$&$  7505.64$&$ 10.5$&$  18.2\pm       0.3$&$4731\pm  42$&$5.22\pm0.14$&$-0.63\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-007&11:49:55.63&-18:07:06.3&$ 19.03$&$ 17.45$&$  7505.64$&$  7.1$&$   3.2\pm       0.4$&$4880\pm  44$&$4.99\pm0.17$&$-0.16\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-008&11:47:26.83&-18:04:41.1&$ 18.89$&$ 17.63$&$  7505.64$&$ 10.1$&$  -3.0\pm       0.3$&$4931\pm  35$&$5.21\pm0.13$&$ 0.02\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-009&11:48:02.16&-18:53:19.5&$ 18.92$&$ 17.53$&$  7505.64$&$  8.9$&$  57.9\pm       0.4$&$4907\pm  39$&$5.27\pm0.16$&$-0.13\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-010&11:48:40.05&-18:26:07.3&$ 19.08$&$ 17.49$&$  7505.64$&$  8.2$&$  -1.1\pm       0.4$&$4821\pm  41$&$5.47\pm0.17$&$-0.09\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-011&11:50:08.07&-18:22:25.2&$ 18.96$&$ 17.58$&$  7505.64$&$  7.7$&$  31.3\pm       0.4$&$4975\pm  44$&$5.10\pm0.17$&$ 0.09\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-012&11:48:17.17&-18:09:37.0&$ 18.83$&$ 17.68$&$  7505.64$&$ 10.3$&$   2.2\pm       0.3$&$5139\pm  38$&$5.52\pm0.14$&$-0.35\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-013&11:47:48.50&-18:29:56.0&$ 19.06$&$ 17.61$&$  7505.64$&$  8.6$&$  17.6\pm       0.4$&$4821\pm  40$&$5.37\pm0.16$&$-0.06\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-014&11:48:22.08&-18:51:25.9&$ 18.98$&$ 17.66$&$  7505.64$&$  8.0$&$ 103.5\pm       0.4$&$4836\pm  41$&$5.00\pm0.15$&$-0.21\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-015&11:49:00.76&-18:21:42.8&$ 19.14$&$ 17.69$&$  7505.64$&$  7.4$&$ 178.2\pm       0.6$&$4985\pm  62$&$5.36\pm0.25$&$-0.81\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-016&11:47:28.72&-18:30:11.6&$ 19.10$&$ 17.78$&$  7505.64$&$  8.7$&$  25.2\pm       0.3$&$4794\pm  36$&$5.05\pm0.12$&$ 0.06\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-017&11:48:35.36&-18:41:30.8&$ 18.99$&$ 17.76$&$  7505.64$&$  5.6$&$  49.8\pm       0.4$&$4947\pm  48$&$5.39\pm0.19$&$-0.13\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-018&11:47:17.36&-18:14:52.3&$ 19.15$&$ 17.80$&$  7505.64$&$  8.4$&$  79.5\pm       0.4$&$4797\pm  40$&$5.14\pm0.14$&$-0.24\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-019&11:50:14.59&-18:25:08.1&$ 19.18$&$ 17.78$&$  7505.64$&$  5.5$&$   6.7\pm       0.5$&$4870\pm  55$&$5.50\pm0.22$&$-0.24\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-020&11:48:41.28&-18:18:20.7&$ 18.96$&$ 17.89$&$  7505.64$&$  8.8$&$  26.4\pm       0.4$&$5152\pm  58$&$5.06\pm0.20$&$-0.40\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-021&11:46:28.03&-18:36:18.2&$ 19.07$&$ 17.89$&$  7505.64$&$  6.3$&$  62.5\pm       0.4$&$5007\pm  53$&$5.41\pm0.20$&$-0.17\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-022&11:47:23.79&-18:35:25.8&$ 19.14$&$ 17.94$&$  7505.64$&$  8.6$&$  51.1\pm       0.4$&$4896\pm  40$&$5.17\pm0.15$&$-0.27\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-023&11:50:04.15&-18:20:04.2&$ 19.06$&$ 17.93$&$  7505.64$&$  6.8$&$ -30.3\pm       0.5$&$5108\pm  74$&$5.04\pm0.24$&$-0.59\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-024&11:47:56.79&-18:11:59.5&$ 19.23$&$ 17.92$&$  7505.64$&$  6.4$&$  32.2\pm       0.4$&$4687\pm  49$&$4.70\pm0.16$&$ 0.05\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-025&11:48:24.75&-18:22:08.5&$ 19.17$&$ 17.90$&$  7505.64$&$  9.0$&$  91.1\pm       0.5$&$4750\pm 100$&$1.28\pm0.24$&$-2.28\pm0.12$\\%$1.000_{-0.000}^{+0.000}$
Cra2-026&11:47:32.40&-18:44:16.4&$ 19.08$&$ 17.82$&$  7505.64$&$  8.6$&$  88.9\pm       0.6$&$4758\pm 104$&$1.12\pm0.17$&$-2.36\pm0.12$\\%$1.000_{-0.000}^{+0.000}$
Cra2-027&11:49:32.51&-18:01:43.3&$ 19.20$&$ 17.97$&$  7505.64$&$  6.6$&$  19.0\pm       0.5$&$5173\pm  61$&$4.95\pm0.19$&$ 0.32\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-028&11:47:03.87&-18:01:14.8&$ 19.16$&$ 17.97$&$  7505.64$&$  6.9$&$  52.8\pm       0.4$&$5037\pm  49$&$5.14\pm0.17$&$-0.02\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-029&11:47:12.06&-18:18:12.9&$ 19.26$&$ 17.99$&$  7505.64$&$  7.7$&$ 152.7\pm       0.4$&$4869\pm  45$&$5.16\pm0.15$&$ 0.06\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-030&11:49:06.84&-18:43:44.7&$ 19.24$&$ 17.92$&$  7505.64$&$  5.4$&$  32.0\pm       0.4$&$4861\pm  51$&$4.90\pm0.18$&$ 0.22\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-031&11:48:29.03&-18:47:59.1&$ 19.08$&$ 18.05$&$  7505.64$&$  8.0$&$  65.8\pm       0.4$&$5151\pm  46$&$5.08\pm0.16$&$-0.11\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-032&11:46:32.45&-18:40:16.1&$ 19.20$&$ 18.06$&$  7505.64$&$  5.7$&$  78.5\pm       0.5$&$4933\pm  70$&$4.97\pm0.23$&$-0.04\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-033&11:49:30.17&-18:12:33.8&$ 19.19$&$ 18.12$&$  7505.64$&$  6.9$&$  19.1\pm       0.5$&$4934\pm  62$&$4.25\pm0.20$&$-0.57\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-034&11:48:39.88&-18:06:38.4&$ 19.12$&$ 18.11$&$  7505.64$&$  8.5$&$  35.0\pm       0.4$&$5253\pm  52$&$4.60\pm0.14$&$-0.12\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-035&11:48:38.59&-17:57:01.0&$ 19.37$&$ 18.10$&$  7505.64$&$  7.8$&$   9.1\pm       0.4$&$4820\pm  53$&$4.51\pm0.19$&$-0.64\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-036&11:48:14.08&-18:25:02.8&$ 19.32$&$ 18.10$&$  7505.64$&$  7.7$&$  87.8\pm       0.5$&$4503\pm  73$&$1.17\pm0.18$&$-2.18\pm0.08$\\%$1.000_{-0.000}^{+0.000}$
Cra2-037&11:48:34.27&-18:32:50.3&$ 19.37$&$ 18.22$&$  7505.64$&$  5.4$&$  86.2\pm       0.4$&$4944\pm  60$&$4.93\pm0.22$&$-0.36\pm0.09$\\%$0.000_{-0.000}^{+0.000}$
Cra2-038&11:47:30.56&-18:39:34.4&$ 19.34$&$ 18.24$&$  7505.64$&$  7.2$&$ -49.3\pm       0.4$&$5005\pm  60$&$5.05\pm0.20$&$-0.65\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-039&11:49:34.62&-18:20:33.7&$ 19.39$&$ 18.19$&$  7505.64$&$  6.5$&$  89.2\pm       0.5$&$4721\pm 110$&$1.30\pm0.24$&$-1.91\pm0.13$\\%$1.000_{-0.000}^{+0.000}$
Cra2-040&11:47:29.79&-18:09:52.3&$ 19.41$&$ 18.26$&$  7505.64$&$  6.7$&$   6.9\pm       0.4$&$5000\pm  57$&$5.16\pm0.20$&$-0.19\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-041&11:48:27.80&-17:57:45.7&$ 19.30$&$ 18.30$&$  7505.64$&$  7.8$&$  18.3\pm       0.4$&$5092\pm  68$&$4.39\pm0.19$&$-0.42\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-042&11:48:14.86&-18:07:42.5&$ 19.39$&$ 18.27$&$  7505.64$&$  6.4$&$ -30.2\pm       0.4$&$4959\pm  57$&$5.30\pm0.19$&$-0.60\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-043&11:48:55.72&-18:08:18.4&$ 19.44$&$ 18.22$&$  7505.64$&$  7.4$&$  87.4\pm       0.6$&$4761\pm 111$&$1.42\pm0.27$&$-2.09\pm0.14$\\%$1.000_{-0.000}^{+0.000}$
Cra2-044&11:47:47.34&-18:32:27.5&$ 19.43$&$ 18.29$&$  7505.64$&$  6.7$&$  73.6\pm       0.5$&$4848\pm  57$&$4.79\pm0.21$&$-0.63\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-045&11:48:08.86&-18:28:07.1&$ 19.38$&$ 18.31$&$  7505.64$&$  7.1$&$  36.3\pm       0.4$&$5005\pm  46$&$4.80\pm0.15$&$ 0.03\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-046&11:46:58.39&-18:33:30.2&$ 19.49$&$ 18.27$&$  7505.64$&$  5.3$&$  67.2\pm       0.5$&$4950\pm  66$&$5.29\pm0.23$&$-0.29\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-047&11:50:03.08&-18:23:36.0&$ 19.54$&$ 18.27$&$  7505.64$&$  5.5$&$  64.5\pm       0.5$&$4985\pm  58$&$5.35\pm0.22$&$-0.28\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-048&11:49:55.17&-18:21:34.5&$ 19.47$&$ 18.35$&$  7505.64$&$  5.5$&$  71.8\pm       0.7$&$5004\pm 107$&$1.21\pm0.24$&$-1.61\pm0.14$\\%$0.001_{-0.001}^{+0.023}$
Cra2-049&11:47:24.54&-18:21:05.2&$ 19.48$&$ 18.38$&$  7505.64$&$  7.0$&$  86.8\pm       0.5$&$4736\pm 120$&$1.44\pm0.29$&$-1.87\pm0.15$\\%$1.000_{-0.000}^{+0.000}$
Cra2-050&11:49:29.02&-18:14:54.9&$ 19.53$&$ 18.35$&$  7505.64$&$  5.7$&$  45.4\pm       0.7$&$5134\pm 104$&$4.76\pm0.32$&$-1.01\pm0.15$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-051&11:47:16.04&-18:32:53.6&$ 18.16$&$ 16.54$&$  7505.64$&$ 16.5$&$  70.2\pm       0.3$&$4660\pm  31$&$5.20\pm0.12$&$-0.51\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-052&11:48:51.52&-18:44:44.2&$ 19.57$&$ 18.36$&$  7505.64$&$  4.5$&$  70.0\pm       0.6$&$4930\pm  82$&$4.68\pm0.29$&$-0.38\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-053&11:50:06.80&-18:10:44.4&$ 19.56$&$ 18.40$&$  7505.64$&$  5.0$&$  88.4\pm       0.8$&$4787\pm 155$&$1.39\pm0.32$&$-2.10\pm0.20$\\%$1.000_{-0.000}^{+0.000}$
Cra2-054&11:47:51.80&-18:35:50.9&$ 19.63$&$ 18.45$&$  7505.64$&$  6.2$&$  74.3\pm       0.5$&$4930\pm  64$&$5.27\pm0.23$&$-0.44\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-055&11:49:59.68&-18:27:44.9&$ 19.54$&$ 18.46$&$  7505.64$&$  4.6$&$  83.0\pm       0.7$&$4576\pm 121$&$1.29\pm0.26$&$-2.32\pm0.14$\\%$1.000_{-0.000}^{+0.000}$
Cra2-056&11:49:28.14&-18:10:40.4&$ 19.46$&$ 18.50$&$  7505.64$&$  6.2$&$ -47.7\pm       0.9$&$5073\pm 134$&$4.30\pm0.34$&$-1.53\pm0.19$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-057&11:48:26.42&-18:49:33.5&$ 18.21$&$ 16.41$&$  7505.64$&$ 15.6$&$  12.8\pm       0.4$&$4722\pm  32$&$5.39\pm0.15$&$-0.07\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-058&11:48:29.83&-18:44:00.7&$ 18.20$&$ 16.43$&$  7505.64$&$ 13.0$&$   1.2\pm       0.3$&$4531\pm  47$&$5.47\pm0.15$&$-0.41\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-059&11:49:19.00&-18:11:45.5&$ 19.55$&$ 18.51$&$  7505.64$&$  6.1$&$  85.0\pm       0.8$&$4937\pm 164$&$1.31\pm0.31$&$-2.22\pm0.21$\\%$1.000_{-0.000}^{+0.000}$
Cra2-060&11:49:29.24&-18:27:46.0&$ 19.66$&$ 18.59$&$  7505.64$&$  4.4$&$ -58.5\pm       0.8$&$5096\pm  65$&$5.38\pm0.25$&$-0.08\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-061&11:48:00.23&-18:19:19.2&$ 19.59$&$ 18.52$&$  7505.64$&$  4.5$&$ 207.2\pm       0.7$&$5051\pm  96$&$5.02\pm0.32$&$-0.82\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-062&11:47:23.94&-18:35:53.6&$ 19.75$&$ 18.56$&$  7505.64$&$  4.5$&$ -51.7\pm       0.5$&$4817\pm  68$&$5.07\pm0.21$&$ 0.05\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-063&11:48:29.14&-18:24:09.3&$ 19.68$&$ 18.52$&$  7505.64$&$  5.1$&$  19.3\pm       0.6$&$5033\pm  66$&$5.25\pm0.25$&$-0.15\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-064&11:48:13.11&-18:47:10.0&$ 19.67$&$ 18.54$&$  7505.64$&$  5.2$&$  86.9\pm       0.7$&$4775\pm 148$&$1.56\pm0.36$&$-1.95\pm0.18$\\%$1.000_{-0.000}^{+0.000}$
Cra2-065&11:48:15.45&-18:45:43.9&$ 19.72$&$ 18.56$&$  7505.64$&$  4.8$&$  63.3\pm       0.5$&$4969\pm  71$&$5.25\pm0.26$&$-0.52\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-066&11:48:40.61&-18:13:43.2&$ 19.61$&$ 18.55$&$  7505.64$&$  5.6$&$  26.0\pm       0.7$&$5352\pm  85$&$5.57\pm0.23$&$-0.94\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-067&11:47:18.62&-18:24:14.4&$ 19.65$&$ 18.60$&$  7505.64$&$  5.7$&$  78.3\pm       0.5$&$5213\pm  63$&$5.54\pm0.21$&$-0.27\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-068&11:47:08.82&-18:05:38.0&$ 19.73$&$ 18.70$&$  7505.64$&$  4.4$&$   6.2\pm       0.6$&$5056\pm  95$&$5.09\pm0.31$&$-0.60\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-069&11:48:19.92&-18:18:54.4&$ 19.80$&$ 18.71$&$  7505.64$&$  5.1$&$   9.0\pm       0.8$&$4664\pm 119$&$3.69\pm0.33$&$-1.74\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-070&11:46:57.79&-18:04:01.3&$ 19.83$&$ 18.77$&$  7505.64$&$  4.1$&$ 160.3\pm       0.7$&$5117\pm  87$&$5.53\pm0.25$&$-0.74\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-071&11:48:51.11&-18:41:59.7&$ 19.85$&$ 18.84$&$  7505.64$&$  3.5$&$  21.9\pm       0.8$&$5169\pm 115$&$5.25\pm0.36$&$-0.61\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-072&11:48:12.86&-18:18:37.3&$ 19.87$&$ 18.85$&$  7505.64$&$  4.8$&$  81.8\pm       1.0$&$5122\pm 240$&$1.66\pm0.51$&$-1.92\pm0.28$\\%$0.999_{-0.001}^{+0.000}$
Cra2-073&11:48:21.07&-18:36:04.0&$ 19.86$&$ 18.77$&$  7505.64$&$  4.7$&$  86.3\pm       0.7$&$4934\pm 148$&$1.73\pm0.39$&$-1.90\pm0.19$\\%$1.000_{-0.000}^{+0.000}$
Cra2-074&11:47:07.10&-18:03:30.5&$ 19.83$&$ 18.89$&$  7505.64$&$  4.2$&$ 173.6\pm       0.8$&$5171\pm 106$&$5.53\pm0.26$&$-1.07\pm0.14$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-075&11:48:18.65&-18:27:54.7&$ 19.89$&$ 18.81$&$  7505.64$&$  2.8$&$  94.5\pm       1.1$&$5066\pm 334$&$2.01\pm0.60$&$-1.75\pm0.40$\\%$0.998_{-0.001}^{+0.001}$
Cra2-076&11:47:33.94&-18:21:29.7&$ 19.87$&$ 18.84$&$  7505.64$&$  4.3$&$  86.6\pm       0.8$&$4795\pm 164$&$1.69\pm0.48$&$-1.75\pm0.21$\\%$1.000_{-0.000}^{+0.000}$
Cra2-077&11:47:22.58&-18:34:53.3&$ 19.87$&$ 18.88$&$  7505.64$&$  4.2$&$  59.4\pm       0.5$&$5036\pm  70$&$4.88\pm0.21$&$ 0.01\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-078&11:48:14.84&-18:12:37.9&$ 19.96$&$ 18.87$&$  7505.64$&$  4.4$&$  22.8\pm       0.8$&$4967\pm  97$&$5.04\pm0.30$&$-0.86\pm0.15$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-079&11:47:10.88&-18:34:44.3&$ 19.88$&$ 18.87$&$  7505.64$&$  4.2$&$ 193.3\pm       0.7$&$5085\pm 113$&$4.90\pm0.33$&$-0.82\pm0.14$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-080&11:47:36.90&-18:50:09.0&$ 19.89$&$ 18.85$&$  7505.64$&$  3.5$&$  85.4\pm       0.9$&$4658\pm 164$&$1.33\pm0.30$&$-2.28\pm0.19$\\%$1.000_{-0.000}^{+0.000}$
Cra2-081&11:48:45.77&-18:15:47.0&$ 19.96$&$ 18.90$&$  7505.64$&$  4.6$&$  74.4\pm       0.8$&$5225\pm 132$&$5.16\pm0.39$&$-1.02\pm0.18$\\%$0.000_{-0.000}^{+0.000}$
Cra2-082&11:47:18.31&-18:33:57.7&$ 19.94$&$ 18.89$&$  7505.64$&$  3.8$&$  87.7\pm       0.8$&$4840\pm 167$&$1.36\pm0.33$&$-1.74\pm0.21$\\%$1.000_{-0.000}^{+0.000}$
Cra2-083&11:47:45.50&-18:21:40.8&$ 19.90$&$ 18.87$&$  7505.64$&$  4.3$&$  85.4\pm       1.1$&$4780\pm 197$&$1.54\pm0.42$&$-2.17\pm0.24$\\%$1.000_{-0.000}^{+0.000}$
Cra2-084&11:48:18.21&-18:35:55.3&$ 19.96$&$ 18.95$&$  7505.64$&$  3.8$&$  77.4\pm       0.8$&$4821\pm 113$&$4.37\pm0.35$&$-0.16\pm0.19$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-085&11:48:04.34&-18:31:25.5&$ 19.97$&$ 19.00$&$  7505.64$&$  4.1$&$  88.2\pm       1.3$&$5015\pm 235$&$1.48\pm0.42$&$-2.29\pm0.27$\\%$1.000_{-0.000}^{+0.000}$
Cra2-086&11:48:50.24&-18:29:57.0&$ 20.02$&$ 19.02$&$  7505.64$&$  4.2$&$  88.1\pm       1.4$&$5012\pm 334$&$1.92\pm0.64$&$-2.31\pm0.40$\\%$1.000_{-0.000}^{+0.000}$
Cra2-087&11:48:05.29&-18:36:12.4&$ 20.04$&$ 19.02$&$  7505.64$&$  4.1$&$  89.0\pm       0.9$&$5093\pm 253$&$1.81\pm0.54$&$-1.97\pm0.29$\\%$1.000_{-0.000}^{+0.000}$
Cra2-088&11:47:38.15&-18:14:56.1&$ 20.08$&$ 19.16$&$  7505.64$&$  4.0$&$ 212.2\pm       0.9$&$5135\pm 137$&$4.87\pm0.41$&$-0.83\pm0.18$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-089&11:50:10.24&-18:28:25.6&$ 19.99$&$ 19.03$&$  7505.64$&$  2.4$&$  83.4\pm       1.6$&$5507\pm 690$&$2.72\pm0.85$&$-1.41\pm0.66$\\%$0.991_{-0.003}^{+0.002}$
Cra2-090&11:47:53.96&-18:41:38.3&$ 20.05$&$ 19.11$&$  7505.64$&$  3.2$&$ -25.0\pm       0.9$&$4938\pm 133$&$4.66\pm0.37$&$-0.68\pm0.18$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-091&11:48:25.96&-18:32:23.5&$ 20.13$&$ 19.09$&$  7505.64$&$  3.1$&$  83.8\pm       1.1$&$5137\pm 407$&$2.00\pm0.59$&$-1.74\pm0.46$\\%$0.999_{-0.000}^{+0.000}$
Cra2-092&11:48:59.69&-18:21:05.3&$ 20.10$&$ 19.10$&$  7505.64$&$  4.5$&$  88.2\pm       1.8$&$4766\pm 342$&$1.79\pm0.60$&$-3.06\pm0.38$\\%$1.000_{-0.000}^{+0.000}$
Cra2-093&11:47:31.62&-18:36:16.1&$ 18.26$&$ 16.69$&$  7505.64$&$ 15.7$&$  -9.8\pm       0.3$&$4778\pm  29$&$5.26\pm0.10$&$ 0.20\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-094&11:47:36.20&-18:44:01.5&$ 20.18$&$ 19.16$&$  7505.64$&$  2.7$&$ 128.0\pm       0.9$&$4652\pm 143$&$4.60\pm0.41$&$-1.08\pm0.18$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-095&11:48:36.05&-18:38:47.2&$ 20.08$&$ 19.26$&$  7505.64$&$  2.8$&$  66.6\pm       2.1$&$5669\pm 520$&$5.01\pm0.61$&$-1.87\pm0.58$\\%$0.000_{-0.000}^{+0.000}$
Cra2-096&11:46:36.06&-18:19:38.9&$ 20.27$&$ 19.25$&$  7505.64$&$  2.2$&$  80.0\pm       1.6$&$5138\pm 191$&$5.11\pm0.47$&$-0.82\pm0.25$\\%$0.000_{-0.000}^{+0.000}$
Cra2-097&11:47:33.68&-18:17:13.8&$ 20.13$&$ 19.28$&$  7505.64$&$  3.1$&$ 309.2\pm       0.8$&$5107\pm 218$&$2.52\pm0.50$&$-0.86\pm0.31$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-098&11:47:29.12&-17:57:05.8&$ 20.24$&$ 19.18$&$  7505.64$&$  3.2$&$  88.2\pm       1.4$&$5409\pm 458$&$2.47\pm0.83$&$-1.51\pm0.48$\\%$0.994_{-0.001}^{+0.001}$
Cra2-099&11:48:48.80&-18:03:29.9&$ 20.29$&$ 19.26$&$  7505.64$&$  5.1$&$  86.4\pm       1.4$&$5333\pm 368$&$1.83\pm0.58$&$-2.15\pm0.40$\\%$1.000_{-0.000}^{+0.000}$
Cra2-100&11:46:50.55&-18:25:11.4&$ 20.42$&$ 19.38$&$  7505.64$&$  1.3$&$  71.2\pm       1.0$&$4670\pm 147$&$4.93\pm0.44$&$ 0.33\pm0.21$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-101&11:47:19.33&-18:04:35.2&$ 20.37$&$ 19.34$&$  7505.64$&$  2.9$&$  28.9\pm       1.1$&$5218\pm 137$&$5.33\pm0.37$&$-0.43\pm0.22$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-102&11:49:28.96&-18:29:39.2&$ 20.25$&$ 19.37$&$  7505.64$&$  2.9$&$  85.0\pm       1.2$&$4655\pm 185$&$1.21\pm0.24$&$-2.20\pm0.25$\\%$1.000_{-0.000}^{+0.000}$
Cra2-103&11:48:33.67&-17:55:11.3&$ 20.23$&$ 19.49$&$  7505.64$&$  3.5$&$ 145.6\pm       1.0$&$5173\pm 207$&$4.47\pm0.50$&$-1.27\pm0.28$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-104&11:48:55.24&-18:02:23.9&$ 20.44$&$ 19.44$&$  7505.64$&$  4.9$&$  77.6\pm       1.2$&$5423\pm 305$&$4.61\pm0.50$&$-1.57\pm0.35$\\%$0.018_{-0.012}^{+0.032}$
Cra2-105&11:46:50.02&-18:32:19.4&$ 20.31$&$ 19.44$&$  7505.64$&$  1.8$&$  94.2\pm       1.5$&$5806\pm1085$&$2.20\pm0.88$&$-1.11\pm0.92$\\%$0.963_{-0.021}^{+0.014}$
Cra2-106&11:48:09.04&-18:53:12.0&$ 20.25$&$ 19.44$&$  7505.64$&$  2.0$&$ 139.2\pm       1.2$&$5166\pm 352$&$2.61\pm0.69$&$-0.76\pm0.42$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-107&11:48:37.37&-18:05:53.6&$ 20.36$&$ 19.43$&$  7505.64$&$  4.4$&$  90.1\pm       1.4$&$5085\pm 320$&$1.66\pm0.53$&$-2.54\pm0.35$\\%$1.000_{-0.000}^{+0.000}$
Cra2-108&11:48:20.50&-18:32:33.4&$ 20.45$&$ 19.45$&$  7505.64$&$  3.1$&$  82.0\pm       1.6$&$5065\pm 398$&$2.18\pm0.75$&$-2.15\pm0.43$\\%$0.998_{-0.001}^{+0.000}$
Cra2-109&11:49:01.09&-18:27:32.8&$ 20.42$&$ 19.51$&$  7505.64$&$  3.2$&$  95.3\pm       1.4$&$5029\pm 358$&$3.89\pm0.78$&$-2.04\pm0.47$\\%$0.950_{-0.037}^{+0.018}$
Cra2-110&11:46:14.09&-18:29:17.2&$ 20.28$&$ 19.58$&$  7505.64$&$  1.4$&$ 130.8\pm       1.4$&$4791\pm 290$&$2.65\pm0.91$&$-1.29\pm0.38$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-111&11:47:51.65&-18:36:49.0&$ 20.35$&$ 19.63$&$  7505.64$&$  3.0$&$ 369.3\pm       1.6$&$5522\pm 538$&$3.64\pm0.95$&$-1.42\pm0.57$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-112&11:49:24.62&-18:37:32.5&$ 20.49$&$ 19.54$&$  7505.64$&$  2.0$&$  86.9\pm       1.4$&$5189\pm 488$&$2.05\pm0.80$&$-1.83\pm0.55$\\%$1.000_{-0.000}^{+0.000}$
Cra2-113&11:47:05.80&-18:48:15.1&$ 20.46$&$ 19.58$&$  7505.64$&$  2.1$&$  55.5\pm       1.5$&$4901\pm 287$&$4.25\pm0.74$&$-1.69\pm0.33$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-114&11:48:13.86&-17:54:41.7&$ 20.55$&$ 19.66$&$  7505.64$&$  2.4$&$ 125.1\pm       1.2$&$5349\pm 199$&$5.14\pm0.47$&$-0.87\pm0.28$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-115&11:48:35.65&-17:56:00.3&$ 20.40$&$ 19.69$&$  7505.64$&$  3.1$&$ 313.3\pm       1.4$&$5720\pm 400$&$4.92\pm0.61$&$-1.24\pm0.42$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-116&11:48:49.70&-18:12:46.5&$ 20.48$&$ 19.59$&$  7505.64$&$  3.0$&$ 123.0\pm       1.1$&$5843\pm 294$&$4.86\pm0.57$&$-0.14\pm0.39$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-117&11:47:15.02&-18:33:40.4&$ 20.40$&$ 19.64$&$  7505.64$&$  2.7$&$ 336.8\pm       2.9$&$5541\pm 492$&$4.74\pm0.99$&$-1.75\pm0.56$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-118&11:48:57.10&-18:46:28.2&$ 18.33$&$ 16.78$&$  7505.64$&$ 12.0$&$  -2.6\pm       0.3$&$4830\pm  32$&$5.34\pm0.13$&$ 0.12\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-119&11:48:01.53&-18:21:39.8&$ 20.70$&$ 19.70$&$  7505.64$&$  1.8$&$  87.9\pm       1.5$&$6020\pm 649$&$1.89\pm0.85$&$-0.78\pm0.59$\\%$0.994_{-0.001}^{+0.001}$
Cra2-120&11:48:01.27&-18:23:30.8&$ 20.65$&$ 19.63$&$  7505.64$&$  2.2$&$  88.1\pm       1.2$&$4834\pm 272$&$2.09\pm0.62$&$-1.71\pm0.35$\\%$1.000_{-0.000}^{+0.000}$
Cra2-121&11:48:22.42&-18:24:20.8&$ 18.31$&$ 16.72$&$  7505.64$&$ 12.7$&$   9.8\pm       0.3$&$4862\pm  31$&$5.12\pm0.12$&$ 0.03\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-122&11:49:16.86&-18:17:54.5&$ 20.68$&$ 19.80$&$  7505.64$&$  3.3$&$  89.9\pm       2.0$&$4943\pm 357$&$1.91\pm0.63$&$-2.48\pm0.41$\\%$1.000_{-0.000}^{+0.000}$
Cra2-123&11:47:15.71&-18:18:09.3&$ 20.64$&$ 19.73$&$  7505.64$&$  2.0$&$ 167.8\pm       1.2$&$4781\pm 202$&$4.30\pm0.64$&$-0.65\pm0.28$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-124&11:49:24.77&-18:31:39.1&$ 20.76$&$ 19.79$&$  7505.64$&$  1.0$&$  85.5\pm       2.1$&$5817\pm 753$&$2.00\pm0.93$&$-0.29\pm0.81$\\%$0.981_{-0.004}^{+0.003}$
Cra2-125&11:49:38.64&-18:30:03.0&$ 20.84$&$ 19.91$&$  7505.64$&$  3.4$&$  88.8\pm       1.9$&$5274\pm 452$&$1.90\pm0.67$&$-2.08\pm0.51$\\%$1.000_{-0.000}^{+0.000}$
Cra2-126&11:47:55.58&-18:04:46.7&$ 20.95$&$ 20.09$&$  7505.64$&$  2.0$&$ 169.4\pm       1.7$&$5308\pm 252$&$5.42\pm0.38$&$-1.07\pm0.35$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-127&11:49:38.60&-18:41:10.1&$ 18.25$&$ 16.92$&$  7505.64$&$ 13.4$&$  28.5\pm       0.3$&$4984\pm  29$&$5.36\pm0.10$&$ 0.16\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-128&11:49:04.61&-18:29:05.0&$ 18.37$&$ 16.78$&$  7505.64$&$ 13.0$&$ -17.2\pm       0.3$&$4763\pm  33$&$4.92\pm0.14$&$-0.21\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-129&11:49:21.98&-18:45:01.5&$ 18.50$&$ 16.84$&$  7505.64$&$ 12.2$&$   1.0\pm       0.3$&$4703\pm  33$&$5.34\pm0.14$&$-0.21\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-130&11:48:24.12&-18:23:17.1&$ 18.42$&$ 16.96$&$  7505.64$&$ 11.3$&$  56.9\pm       0.4$&$4895\pm  36$&$5.21\pm0.15$&$-0.15\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-131&11:50:04.38&-18:29:15.7&$ 18.26$&$ 17.05$&$  7505.64$&$ 11.5$&$ -20.7\pm       0.3$&$4996\pm  32$&$5.12\pm0.11$&$ 0.11\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-132&11:48:59.35&-18:39:24.0&$ 18.60$&$ 16.93$&$  7505.64$&$ 10.5$&$  47.4\pm       0.4$&$4433\pm  31$&$4.98\pm0.15$&$-1.34\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-133&11:48:07.66&-18:27:42.4&$ 18.34$&$ 17.04$&$  7505.64$&$ 15.6$&$ 321.1\pm       0.3$&$4787\pm  36$&$5.47\pm0.12$&$-1.34\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-134&11:47:59.21&-18:10:40.5&$ 18.47$&$ 16.94$&$  7505.64$&$ 13.1$&$  85.8\pm       0.4$&$4496\pm  58$&$1.03\pm0.10$&$-2.14\pm0.06$\\%$1.000_{-0.000}^{+0.000}$
Cra2-135&11:50:08.68&-18:18:14.6&$ 18.42$&$ 17.02$&$  7505.64$&$ 11.7$&$  83.1\pm       0.4$&$4802\pm  55$&$1.06\pm0.12$&$-1.75\pm0.07$\\%$1.000_{-0.000}^{+0.000}$
Cra2-136&11:47:35.60&-18:22:08.5&$ 18.67$&$ 17.02$&$  7505.64$&$ 11.7$&$  87.8\pm       0.3$&$4483\pm  53$&$1.03\pm0.10$&$-1.41\pm0.05$\\%$0.997_{-0.006}^{+0.002}$
Cra2-137&11:49:32.67&-18:10:15.4&$ 18.50$&$ 17.09$&$  7505.64$&$ 11.3$&$  62.0\pm       0.3$&$4810\pm  34$&$5.13\pm0.13$&$-0.33\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-138&11:50:05.86&-18:21:59.3&$ 18.57$&$ 17.09$&$  7505.64$&$  9.7$&$  98.0\pm       0.3$&$4761\pm  37$&$4.97\pm0.14$&$-0.13\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-139&11:48:49.84&-18:30:44.8&$ 18.43$&$ 17.17$&$  7505.64$&$ 12.6$&$   7.9\pm       0.3$&$4918\pm  29$&$4.79\pm0.10$&$ 0.29\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-140&11:47:44.78&-18:35:09.2&$ 18.41$&$ 17.18$&$  7505.64$&$ 13.9$&$  19.4\pm       0.3$&$5101\pm  30$&$5.07\pm0.09$&$ 0.41\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-141&11:50:00.18&-18:12:46.0&$ 18.52$&$ 17.20$&$  7505.64$&$ 10.4$&$  -9.4\pm       0.3$&$4928\pm  31$&$5.07\pm0.11$&$ 0.09\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-142&11:48:57.95&-18:14:31.3&$ 18.49$&$ 17.19$&$  7505.64$&$ 10.7$&$ -28.1\pm       0.3$&$5038\pm  35$&$5.30\pm0.12$&$ 0.04\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-143&11:49:07.69&-18:01:49.6&$ 18.62$&$ 17.11$&$  7505.64$&$ 11.5$&$ -73.0\pm       0.3$&$4841\pm  35$&$5.32\pm0.15$&$-0.40\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-144&11:49:36.92&-18:45:45.9&$ 18.62$&$ 17.14$&$  7505.64$&$ 11.3$&$  90.9\pm       0.6$&$4564\pm  94$&$1.18\pm0.19$&$-1.78\pm0.10$\\%$1.000_{-0.000}^{+0.000}$
Cra2-145&11:49:26.52&-18:36:40.9&$ 18.54$&$ 17.19$&$  7505.64$&$ 11.3$&$  23.0\pm       0.3$&$4853\pm  31$&$5.05\pm0.11$&$ 0.09\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-146&11:47:42.92&-18:16:57.9&$ 18.77$&$ 17.12$&$  7505.64$&$ 10.6$&$  72.9\pm       0.3$&$4599\pm  41$&$5.07\pm0.15$&$-0.03\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-147&11:48:04.59&-18:13:00.4&$ 18.47$&$ 17.27$&$  7505.64$&$ 11.8$&$ -12.9\pm       0.3$&$5002\pm  35$&$5.03\pm0.12$&$-0.29\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-148&11:47:37.98&-18:44:10.0&$ 18.51$&$ 17.28$&$  7505.64$&$ 10.7$&$  50.7\pm       0.3$&$4952\pm  33$&$5.06\pm0.11$&$ 0.32\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-149&11:49:14.18&-18:47:15.0&$ 18.55$&$ 17.35$&$  7505.64$&$  9.8$&$  57.8\pm       0.3$&$5042\pm  38$&$5.19\pm0.13$&$ 0.10\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-150&11:48:34.27&-18:11:20.2&$ 18.53$&$ 17.35$&$  7505.64$&$ 11.1$&$   7.4\pm       0.4$&$5133\pm  38$&$5.24\pm0.13$&$-0.03\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-151&11:48:59.05&-18:29:13.1&$ 18.82$&$ 17.19$&$  7505.64$&$ 10.3$&$  39.2\pm       0.3$&$4765\pm  35$&$5.24\pm0.14$&$-0.12\pm0.04$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-152&11:48:05.07&-18:44:09.4&$ 18.72$&$ 17.18$&$  7505.64$&$ 11.5$&$  90.5\pm       0.4$&$4634\pm  69$&$1.26\pm0.16$&$-1.78\pm0.08$\\%$1.000_{-0.000}^{+0.000}$
Cra2-153&11:47:35.38&-18:02:53.9&$ 18.81$&$ 17.30$&$  7505.64$&$  9.8$&$ -23.9\pm       0.4$&$4766\pm  38$&$5.40\pm0.16$&$-0.33\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-154&11:47:09.65&-18:30:50.5&$ 18.74$&$ 17.33$&$  7505.64$&$ 10.3$&$  89.3\pm       0.4$&$4631\pm  79$&$1.26\pm0.19$&$-1.95\pm0.09$\\%$1.000_{-0.000}^{+0.000}$
Cra2-155&11:48:01.85&-18:51:08.6&$ 18.85$&$ 17.36$&$  7505.64$&$  9.6$&$  -4.6\pm       0.4$&$4844\pm  44$&$5.14\pm0.21$&$-0.40\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-156&11:47:23.13&-18:28:10.4&$ 18.83$&$ 17.43$&$  7505.64$&$ 10.1$&$  47.7\pm       0.3$&$4753\pm  38$&$5.32\pm0.14$&$-0.19\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-157&11:47:48.77&-18:32:59.1&$ 18.84$&$ 17.43$&$  7505.64$&$ 10.1$&$ -17.1\pm       0.3$&$4778\pm  35$&$5.09\pm0.11$&$ 0.32\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-158&11:48:09.71&-18:46:57.3&$ 18.64$&$ 17.49$&$  7505.64$&$ 10.7$&$  17.4\pm       0.3$&$5041\pm  37$&$4.92\pm0.12$&$ 0.37\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-159&11:48:56.03&-18:49:52.7&$ 18.93$&$ 17.37$&$  7505.64$&$  8.3$&$  47.6\pm       0.4$&$4618\pm  52$&$5.37\pm0.17$&$-0.40\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-160&11:49:40.73&-18:12:36.8&$ 18.87$&$ 17.46$&$  7505.64$&$  8.6$&$  67.0\pm       0.4$&$4827\pm  40$&$5.20\pm0.17$&$-0.49\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-161&11:50:47.29&-18:00:46.3&$ 18.91$&$ 17.43$&$  7508.64$&$  7.5$&$  88.8\pm       0.6$&$5135\pm 116$&$2.10\pm0.28$&$-1.50\pm0.16$\\%$0.996_{-0.004}^{+0.002}$
Cra2-162&11:49:56.95&-18:52:12.6&$ 19.01$&$ 17.48$&$  7508.64$&$  3.8$&$ 170.9\pm       1.0$&$4634\pm  94$&$5.78\pm0.10$&$-0.65\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-163&11:50:37.08&-18:16:07.8&$ 18.94$&$ 17.64$&$  7508.64$&$  6.4$&$  89.8\pm       1.0$&$5515\pm 296$&$2.14\pm0.54$&$-1.83\pm0.30$\\%$1.000_{-0.000}^{+0.000}$
Cra2-164&11:51:21.85&-18:34:19.8&$ 19.05$&$ 17.66$&$  7508.64$&$  6.0$&$  49.3\pm       0.7$&$5194\pm  81$&$5.47\pm0.26$&$-0.90\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-165&11:49:19.35&-18:28:48.8&$ 19.03$&$ 17.66$&$  7508.64$&$  5.3$&$  56.4\pm       0.5$&$4677\pm  75$&$5.08\pm0.23$&$-0.71\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-166&11:50:26.35&-18:13:09.5&$ 18.91$&$ 17.68$&$  7508.64$&$  5.5$&$  67.3\pm       0.7$&$5178\pm 101$&$4.79\pm0.33$&$-0.82\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-167&11:51:35.67&-18:35:19.6&$ 19.02$&$ 17.76$&$  7508.64$&$  3.7$&$ 119.6\pm       0.5$&$4951\pm  69$&$5.02\pm0.24$&$ 0.50\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-168&11:49:51.91&-18:41:12.6&$ 19.15$&$ 17.80$&$  7508.64$&$  2.9$&$ -11.5\pm       0.5$&$4572\pm  89$&$4.85\pm0.27$&$ 0.45\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-169&11:51:41.54&-18:12:00.6&$ 19.05$&$ 17.91$&$  7508.64$&$  4.2$&$  18.2\pm       0.8$&$5292\pm  91$&$5.41\pm0.29$&$-0.41\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-170&11:51:52.85&-18:13:58.4&$ 18.98$&$ 17.94$&$  7508.64$&$  4.8$&$  31.6\pm       0.6$&$5519\pm 106$&$5.09\pm0.28$&$-0.06\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-171&11:50:19.65&-18:35:04.0&$ 19.23$&$ 17.83$&$  7508.64$&$  2.9$&$  10.1\pm       0.8$&$5039\pm  86$&$5.38\pm0.31$&$-0.07\pm0.14$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-172&11:49:17.06&-18:34:21.7&$ 19.06$&$ 18.04$&$  7508.64$&$  6.0$&$  57.8\pm       0.5$&$5007\pm  75$&$4.57\pm0.26$&$-0.58\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-173&11:50:45.88&-18:32:07.5&$ 19.08$&$ 18.01$&$  7508.64$&$  2.0$&$  29.8\pm       0.5$&$4800\pm 105$&$4.35\pm0.29$&$ 0.75\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-174&11:50:26.86&-18:19:56.7&$ 19.10$&$ 17.97$&$  7508.64$&$  5.9$&$  64.9\pm       1.0$&$4990\pm 132$&$4.34\pm0.34$&$-1.78\pm0.19$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-175&11:49:35.51&-18:22:37.4&$ 19.05$&$ 18.02$&$  7508.64$&$  5.9$&$  13.4\pm       0.7$&$5163\pm  88$&$5.41\pm0.28$&$-0.94\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-176&11:50:49.71&-18:41:54.7&$ 19.15$&$ 17.98$&$  7508.64$&$  1.9$&$  66.7\pm       0.9$&$4993\pm  99$&$5.33\pm0.32$&$ 0.56\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-177&11:49:55.35&-18:32:12.2&$ 19.22$&$ 17.98$&$  7508.64$&$  3.1$&$ -22.6\pm       0.6$&$4571\pm  89$&$4.70\pm0.25$&$ 0.24\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-178&11:49:12.28&-18:32:05.9&$ 19.24$&$ 17.98$&$  7508.64$&$  4.2$&$  61.9\pm       0.5$&$4741\pm  75$&$4.93\pm0.24$&$-0.34\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-179&11:48:36.37&-18:42:02.9&$ 19.14$&$ 18.05$&$  7508.64$&$  3.3$&$  10.6\pm       0.5$&$4629\pm  99$&$4.68\pm0.29$&$-0.08\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-180&11:49:13.39&-18:21:23.3&$ 19.29$&$ 18.01$&$  7508.64$&$  4.3$&$  72.8\pm       0.6$&$4834\pm  78$&$4.80\pm0.29$&$-0.25\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-181&11:49:19.16&-18:16:58.3&$ 19.24$&$ 17.96$&$  7508.64$&$  4.4$&$  83.0\pm       0.9$&$5044\pm 210$&$2.26\pm0.48$&$-1.71\pm0.27$\\%$0.999_{-0.000}^{+0.000}$
Cra2-182&11:51:36.68&-18:27:20.0&$ 19.17$&$ 18.13$&$  7508.64$&$  3.6$&$  15.6\pm       0.6$&$5213\pm  83$&$5.23\pm0.28$&$-0.28\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-183&11:49:21.74&-18:49:34.9&$ 19.28$&$ 18.12$&$  7508.64$&$  1.8$&$  27.8\pm       0.7$&$4570\pm 114$&$4.66\pm0.39$&$ 0.68\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-184&11:48:20.95&-18:22:34.1&$ 19.21$&$ 18.15$&$  7508.64$&$  5.9$&$  31.6\pm       1.0$&$5332\pm 184$&$4.79\pm0.36$&$-1.30\pm0.21$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-185&11:48:18.14&-18:24:00.7&$ 19.31$&$ 18.16$&$  7508.64$&$  3.7$&$  54.0\pm       0.7$&$5056\pm 101$&$5.26\pm0.32$&$-0.59\pm0.14$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-186&11:50:01.91&-18:44:08.3&$ 19.40$&$ 18.18$&$  7508.64$&$  0.9$&$ -41.2\pm       1.0$&$4674\pm 162$&$4.79\pm0.56$&$ 1.07\pm0.28$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-187&11:50:34.90&-18:18:56.5&$ 19.45$&$ 18.21$&$  7508.64$&$  4.0$&$ 177.4\pm       1.2$&$4639\pm 133$&$4.46\pm0.42$&$-1.99\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-188&11:50:18.51&-18:25:13.3&$ 19.24$&$ 18.24$&$  7508.64$&$  6.7$&$  44.5\pm       1.0$&$5998\pm 386$&$4.66\pm0.58$&$-1.30\pm0.35$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-189&11:51:42.26&-18:39:21.1&$ 19.47$&$ 18.25$&$  7508.64$&$  0.4$&$  55.0\pm       1.6$&$4723\pm 176$&$5.31\pm0.42$&$-0.03\pm0.29$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-190&11:50:37.32&-18:40:34.1&$ 19.41$&$ 18.21$&$  7508.64$&$  1.2$&$  31.2\pm       1.0$&$4967\pm 139$&$5.11\pm0.40$&$ 0.76\pm0.24$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-191&11:48:44.51&-18:31:39.1&$ 19.30$&$ 18.35$&$  7508.64$&$  5.1$&$ -19.3\pm       0.6$&$5394\pm 105$&$5.24\pm0.29$&$-0.33\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-192&11:50:10.67&-18:18:58.2&$ 19.52$&$ 18.25$&$  7508.64$&$  3.8$&$  77.6\pm       0.8$&$4715\pm 124$&$4.23\pm0.41$&$-1.08\pm0.18$\\%$0.001_{-0.000}^{+0.002}$
Cra2-193&11:48:55.53&-18:31:56.6&$ 19.36$&$ 18.29$&$  7508.64$&$  4.3$&$ 196.3\pm       0.7$&$5184\pm  92$&$5.60\pm0.22$&$-1.03\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-194&11:51:15.12&-18:14:29.1&$ 19.37$&$ 18.32$&$  7508.64$&$  4.9$&$  92.4\pm       0.9$&$5175\pm 156$&$4.28\pm0.40$&$-1.43\pm0.21$\\%$0.407_{-0.179}^{+0.169}$
Cra2-195&11:51:18.30&-18:02:45.0&$ 19.36$&$ 18.36$&$  7508.64$&$  3.5$&$  49.0\pm       0.8$&$5578\pm 135$&$5.32\pm0.36$&$-0.27\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-196&11:49:11.70&-18:22:28.2&$ 19.44$&$ 18.36$&$  7508.64$&$  3.5$&$  51.9\pm       0.7$&$4859\pm  96$&$4.65\pm0.33$&$-0.44\pm0.15$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-197&11:51:08.53&-18:34:52.8&$ 19.52$&$ 18.38$&$  7508.64$&$  0.9$&$  31.9\pm       0.7$&$5102\pm 142$&$5.12\pm0.40$&$ 1.34\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-198&11:49:17.45&-18:37:56.8&$ 19.52$&$ 18.40$&$  7508.64$&$  2.2$&$  91.2\pm       1.2$&$4633\pm 158$&$1.19\pm0.24$&$-1.70\pm0.22$\\%$1.000_{-0.000}^{+0.000}$
Cra2-199&11:49:05.30&-18:29:12.7&$ 19.54$&$ 18.39$&$  7508.64$&$  2.4$&$  85.0\pm       1.1$&$4593\pm 144$&$1.29\pm0.29$&$-1.73\pm0.19$\\%$1.000_{-0.000}^{+0.000}$
Cra2-200&11:51:13.31&-18:36:30.0&$ 19.60$&$ 18.41$&$  7508.64$&$  4.1$&$  84.2\pm       1.1$&$5073\pm 360$&$2.13\pm0.61$&$-2.22\pm0.43$\\%$0.999_{-0.000}^{+0.000}$
Cra2-201&11:50:31.29&-18:42:39.4&$ 19.68$&$ 18.44$&$  7508.64$&$  1.1$&$  65.9\pm       0.9$&$5040\pm 137$&$5.33\pm0.38$&$ 0.30\pm0.23$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-202&11:51:52.04&-18:32:56.3&$ 19.59$&$ 18.54$&$  7508.64$&$  1.0$&$  29.8\pm       1.2$&$5330\pm 148$&$5.33\pm0.36$&$ 0.84\pm0.30$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-203&11:49:38.50&-18:50:58.7&$ 19.57$&$ 18.56$&$  7508.64$&$  3.6$&$ -22.6\pm       0.8$&$4798\pm 126$&$4.11\pm0.43$&$-1.24\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-204&11:49:39.90&-18:21:41.5&$ 19.66$&$ 18.50$&$  7508.64$&$  3.2$&$ 133.8\pm       1.1$&$4740\pm 152$&$4.97\pm0.43$&$-1.32\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-205&11:49:40.98&-18:23:43.7&$ 19.54$&$ 18.60$&$  7508.64$&$  3.4$&$ 104.4\pm       0.8$&$4993\pm 120$&$4.15\pm0.34$&$-0.61\pm0.19$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-206&11:50:44.90&-18:10:46.1&$ 19.66$&$ 18.62$&$  7508.64$&$  4.0$&$  86.9\pm       1.8$&$5885\pm 835$&$2.22\pm0.91$&$-1.99\pm0.72$\\%$0.999_{-0.000}^{+0.000}$
Cra2-207&11:48:41.63&-18:35:56.3&$ 19.76$&$ 18.62$&$  7508.64$&$  0.5$&$  25.9\pm       1.6$&$4620\pm 152$&$4.66\pm0.65$&$ 0.87\pm0.29$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-208&11:51:05.17&-18:20:20.3&$ 19.79$&$ 18.64$&$  7508.64$&$  4.0$&$   3.2\pm       1.1$&$6893\pm 898$&$4.10\pm0.87$&$-0.59\pm0.74$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-209&11:51:40.26&-18:38:36.4&$ 19.66$&$ 18.72$&$  7508.64$&$  1.1$&$ -40.5\pm       1.4$&$5213\pm 215$&$4.77\pm0.63$&$-0.00\pm0.32$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-210&11:51:00.96&-18:22:25.8&$ 18.08$&$ 16.66$&$  7508.64$&$  9.2$&$ -18.3\pm       0.4$&$4879\pm  49$&$4.84\pm0.21$&$-0.40\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-211&11:48:32.69&-18:38:57.2&$ 19.75$&$ 18.65$&$  7508.64$&$  3.0$&$  86.5\pm       1.2$&$4825\pm 232$&$1.53\pm0.44$&$-1.87\pm0.29$\\%$1.000_{-0.000}^{+0.000}$
Cra2-212&11:48:54.82&-18:22:03.0&$ 19.64$&$ 18.75$&$  7508.64$&$  4.5$&$ 238.3\pm       1.2$&$5589\pm 217$&$5.42\pm0.35$&$-1.40\pm0.24$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-213&11:51:09.55&-18:26:09.9&$ 18.07$&$ 16.69$&$  7508.64$&$  9.6$&$ -38.4\pm       0.4$&$4903\pm  35$&$4.84\pm0.12$&$ 0.24\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-214&11:50:57.02&-18:22:06.5&$ 19.71$&$ 18.72$&$  7508.64$&$  4.2$&$  85.2\pm       1.9$&$6315\pm 851$&$2.87\pm1.06$&$-1.79\pm0.70$\\%$0.996_{-0.001}^{+0.001}$
Cra2-215&11:49:10.89&-18:30:24.1&$ 19.67$&$ 18.76$&$  7508.64$&$  2.7$&$  91.5\pm       1.1$&$5323\pm 148$&$5.47\pm0.32$&$-0.59\pm0.24$\\%$0.000_{-0.000}^{+0.001}$
Cra2-216&11:50:10.31&-18:47:49.4&$ 18.11$&$ 16.63$&$  7508.64$&$  8.4$&$ -12.8\pm       0.8$&$4537\pm  87$&$4.88\pm0.31$&$ 0.38\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-217&11:51:12.25&-18:47:38.2&$ 19.74$&$ 18.78$&$  7508.64$&$  0.7$&$ 171.7\pm       1.4$&$5146\pm 330$&$4.01\pm0.92$&$ 0.43\pm0.50$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-218&11:50:56.47&-18:05:17.5&$ 18.16$&$ 16.62$&$  7508.64$&$  9.3$&$  26.1\pm       0.4$&$4927\pm  40$&$5.26\pm0.19$&$-0.27\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-219&11:51:17.05&-18:05:11.4&$ 19.70$&$ 18.81$&$  7508.64$&$  4.4$&$ -21.8\pm       1.7$&$4770\pm 300$&$1.93\pm0.59$&$-2.95\pm0.35$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-220&11:49:22.14&-18:30:48.3&$ 19.76$&$ 18.73$&$  7508.64$&$  3.5$&$  89.7\pm       1.5$&$5112\pm 476$&$1.72\pm0.63$&$-2.22\pm0.47$\\%$1.000_{-0.000}^{+0.000}$
Cra2-221&11:50:01.21&-18:18:42.9&$ 19.84$&$ 18.77$&$  7508.64$&$  2.7$&$  58.9\pm       0.9$&$5232\pm 145$&$5.16\pm0.40$&$-0.34\pm0.23$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-222&11:49:49.70&-18:38:32.9&$ 18.06$&$ 16.64$&$  7508.64$&$ 10.7$&$  43.7\pm       0.3$&$4798\pm  34$&$5.13\pm0.12$&$ 0.11\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-223&11:49:10.70&-18:45:50.7&$ 19.77$&$ 18.83$&$  7508.64$&$  1.3$&$ 332.7\pm       2.8$&$5168\pm 401$&$4.86\pm0.86$&$-1.68\pm0.50$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-224&11:49:09.55&-18:03:39.4&$ 19.84$&$ 18.81$&$  7508.64$&$  4.1$&$  82.9\pm       1.6$&$5025\pm 270$&$5.29\pm0.42$&$-2.02\pm0.38$\\%$0.678_{-0.070}^{+0.055}$
Cra2-225&11:48:50.93&-18:45:50.3&$ 19.77$&$ 18.84$&$  7508.64$&$  3.3$&$  22.5\pm       1.1$&$5321\pm 148$&$5.47\pm0.32$&$-0.99\pm0.19$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-226&11:49:56.32&-18:24:59.5&$ 19.98$&$ 18.79$&$  7508.64$&$  2.3$&$  35.0\pm       1.3$&$5398\pm 172$&$5.34\pm0.37$&$-0.29\pm0.24$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-227&11:50:17.29&-18:41:51.2&$ 18.23$&$ 16.63$&$  7508.64$&$  7.3$&$   8.4\pm       0.4$&$4815\pm  40$&$5.35\pm0.18$&$ 0.26\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-228&11:49:55.94&-18:29:41.7&$ 19.91$&$ 18.81$&$  7508.64$&$  1.2$&$  89.7\pm       1.6$&$5531\pm 689$&$2.40\pm1.02$&$-0.33\pm0.67$\\%$0.958_{-0.012}^{+0.010}$
Cra2-229&11:48:29.90&-18:24:02.3&$ 19.99$&$ 18.91$&$  7508.64$&$  3.8$&$  85.3\pm       2.1$&$7309\pm 792$&$3.39\pm1.06$&$-0.96\pm0.63$\\%$0.948_{-0.010}^{+0.008}$
Cra2-230&11:50:05.72&-18:08:51.9&$ 19.93$&$ 19.02$&$  7508.64$&$  4.3$&$ 196.9\pm       1.4$&$5951\pm 344$&$5.00\pm0.52$&$-1.14\pm0.32$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-231&11:48:17.18&-18:24:26.9&$ 20.05$&$ 19.00$&$  7508.64$&$  1.8$&$  87.6\pm       2.2$&$4969\pm 576$&$2.58\pm0.96$&$-1.76\pm0.61$\\%$0.999_{-0.000}^{+0.000}$
Cra2-232&11:50:12.20&-18:53:26.0&$ 18.26$&$ 16.63$&$  7508.64$&$  7.1$&$  19.6\pm       0.4$&$4509\pm  51$&$5.26\pm0.16$&$ 0.28\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-233&11:48:29.72&-18:23:28.3&$ 20.09$&$ 19.04$&$  7508.64$&$  2.9$&$  83.8\pm       2.3$&$7226\pm 809$&$4.47\pm0.96$&$-0.31\pm0.66$\\%$0.094_{-0.020}^{+0.024}$
Cra2-234&11:48:29.67&-18:08:01.7&$ 19.97$&$ 19.15$&$  7508.64$&$  2.0$&$ 109.0\pm       1.3$&$5002\pm 199$&$4.35\pm0.46$&$-0.69\pm0.29$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-235&11:50:29.37&-18:12:50.2&$ 20.04$&$ 19.22$&$  7508.64$&$  4.9$&$ 109.5\pm       1.3$&$6099\pm 774$&$3.04\pm0.90$&$-1.61\pm0.68$\\%$0.000_{-0.000}^{+0.000}$
Cra2-236&11:49:25.68&-18:37:06.7&$ 20.24$&$ 19.12$&$  7508.64$&$  0.8$&$  37.8\pm       2.5$&$4850\pm 319$&$4.88\pm0.72$&$ 0.08\pm0.46$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-237&11:50:44.07&-18:28:59.0&$ 18.15$&$ 16.66$&$  7508.64$&$  6.7$&$  29.7\pm       0.4$&$4806\pm  43$&$4.99\pm0.16$&$ 0.06\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-238&11:48:18.25&-18:38:01.2&$ 20.15$&$ 19.24$&$  7508.64$&$  3.8$&$  78.5\pm       1.2$&$5905\pm 321$&$5.19\pm0.43$&$-1.10\pm0.33$\\%$0.001_{-0.001}^{+0.002}$
Cra2-239&11:51:17.60&-18:40:22.6&$ 20.27$&$ 19.22$&$  7508.64$&$  1.9$&$  81.1\pm       1.6$&$6145\pm 438$&$5.26\pm0.49$&$-0.37\pm0.46$\\%$0.000_{-0.000}^{+0.000}$
Cra2-240&11:50:27.16&-18:43:29.2&$ 18.31$&$ 16.84$&$  7508.64$&$  6.2$&$   3.8\pm       0.4$&$4660\pm  51$&$5.20\pm0.21$&$-0.10\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-241&11:50:27.32&-18:41:58.6&$ 18.23$&$ 16.87$&$  7508.64$&$  6.0$&$  24.2\pm       0.4$&$4713\pm  52$&$5.29\pm0.17$&$ 0.24\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-242&11:50:46.80&-18:46:11.7&$ 18.23$&$ 16.88$&$  7508.64$&$  6.5$&$ 102.6\pm       0.4$&$4845\pm  41$&$4.98\pm0.14$&$ 0.28\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-243&11:51:46.18&-18:12:27.0&$ 18.42$&$ 16.85$&$  7508.64$&$ 10.6$&$ -20.4\pm       1.0$&$4603\pm 106$&$4.27\pm0.31$&$-2.59\pm0.14$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-244&11:49:44.65&-18:19:17.2&$ 18.21$&$ 16.90$&$  7508.64$&$ 10.7$&$  15.1\pm       0.5$&$4899\pm  47$&$5.60\pm0.17$&$-1.02\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-245&11:51:47.61&-18:24:27.5&$ 18.35$&$ 16.89$&$  7508.64$&$  6.3$&$ -48.8\pm       0.4$&$4913\pm  45$&$5.47\pm0.20$&$ 0.02\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-246&11:50:40.34&-18:39:59.6&$ 18.42$&$ 16.87$&$  7508.64$&$  4.5$&$  27.3\pm       0.4$&$4595\pm  66$&$4.89\pm0.20$&$ 0.59\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-247&11:51:08.89&-18:38:09.4&$ 18.21$&$ 16.95$&$  7508.64$&$  8.9$&$  -6.8\pm       0.4$&$5105\pm  42$&$5.25\pm0.14$&$ 0.17\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-248&11:50:35.89&-18:21:47.1&$ 18.50$&$ 16.85$&$  7508.64$&$  8.9$&$  27.2\pm       1.0$&$4520\pm  79$&$4.58\pm0.30$&$-2.40\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-249&11:49:54.68&-18:03:03.9&$ 18.27$&$ 16.94$&$  7508.64$&$  9.2$&$  48.9\pm       0.4$&$4970\pm  44$&$5.36\pm0.17$&$-0.43\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-250&11:51:28.76&-18:13:03.6&$ 18.30$&$ 16.96$&$  7508.64$&$ 10.7$&$  -9.0\pm       1.2$&$4730\pm  82$&$5.43\pm0.31$&$-2.77\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-251&11:51:40.48&-18:16:24.2&$ 18.48$&$ 16.87$&$  7508.64$&$  7.1$&$   4.6\pm       0.4$&$4839\pm  46$&$5.09\pm0.22$&$-0.26\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-252&11:51:47.14&-18:25:53.9&$ 18.47$&$ 17.02$&$  7508.64$&$  5.5$&$  36.7\pm       0.4$&$4812\pm  49$&$5.50\pm0.19$&$ 0.04\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-253&11:51:09.10&-18:16:55.3&$ 18.36$&$ 17.06$&$  7508.64$&$  7.1$&$   3.7\pm       0.5$&$5021\pm  51$&$4.99\pm0.21$&$-0.21\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-254&11:49:58.56&-18:01:55.4&$ 18.35$&$ 17.16$&$  7508.64$&$  9.4$&$ -33.1\pm       0.6$&$4945\pm  65$&$4.86\pm0.23$&$-1.31\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-255&11:51:16.27&-18:09:39.8&$ 18.55$&$ 17.08$&$  7508.64$&$  8.2$&$  52.6\pm       0.5$&$4996\pm  68$&$4.82\pm0.27$&$-0.83\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-256&11:50:42.02&-18:44:46.8&$ 18.67$&$ 17.00$&$  7508.64$&$  3.7$&$  34.8\pm       0.4$&$4550\pm  67$&$5.10\pm0.19$&$ 0.43\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-257&11:50:58.75&-18:35:35.7&$ 18.43$&$ 17.25$&$  7508.64$&$  7.3$&$  37.3\pm       0.4$&$5092\pm  51$&$5.24\pm0.20$&$-0.22\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-258&11:50:15.26&-18:31:28.5&$ 18.51$&$ 17.27$&$  7508.64$&$  5.3$&$  22.2\pm       0.4$&$4853\pm  48$&$5.13\pm0.16$&$ 0.40\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-259&11:51:32.00&-18:15:25.9&$ 18.59$&$ 17.28$&$  7508.64$&$  7.5$&$  19.3\pm       0.7$&$4896\pm  93$&$4.38\pm0.31$&$-1.25\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-260&11:50:21.78&-18:03:48.3&$ 18.78$&$ 17.23$&$  7508.64$&$  8.4$&$  22.8\pm       0.5$&$4705\pm  67$&$5.10\pm0.33$&$-1.32\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-261&11:50:21.31&-18:30:23.4&$ 18.87$&$ 17.30$&$  7508.64$&$  2.7$&$   6.6\pm       0.6$&$4755\pm  72$&$5.63\pm0.18$&$ 0.91\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-262&11:49:35.92&-18:19:02.1&$ 18.52$&$ 17.36$&$  7508.64$&$  7.8$&$   4.8\pm       0.4$&$4946\pm  47$&$5.34\pm0.16$&$-0.59\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-263&11:50:08.21&-18:50:21.2&$ 18.93$&$ 17.26$&$  7508.64$&$  4.6$&$  38.2\pm       0.5$&$4618\pm  63$&$5.33\pm0.25$&$ 0.32\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-264&11:51:02.10&-18:15:36.8&$ 18.70$&$ 17.45$&$  7508.64$&$  6.4$&$  86.9\pm       0.6$&$5024\pm  72$&$4.67\pm0.25$&$-0.73\pm0.12$\\%$0.000_{-0.000}^{+0.000}$
Cra2-265&11:50:41.87&-18:04:30.0&$ 18.99$&$ 17.27$&$  7508.64$&$  6.6$&$  -5.4\pm       0.6$&$4865\pm  75$&$4.18\pm0.26$&$-0.95\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-266&11:50:06.67&-18:10:38.6&$ 18.81$&$ 17.39$&$  7508.64$&$  7.7$&$  89.1\pm       0.8$&$4940\pm 155$&$1.77\pm0.37$&$-2.03\pm0.20$\\%$1.000_{-0.000}^{+0.000}$
Cra2-267&11:53:52.93&-18:16:56.5&$ 18.65$&$ 17.55$&$  7519.65$&$  6.7$&$  33.6\pm       0.5$&$5072\pm  70$&$4.40\pm0.21$&$-0.62\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-268&11:53:42.05&-18:24:08.1&$ 18.85$&$ 17.46$&$  7519.65$&$  6.0$&$   8.7\pm       0.6$&$5005\pm  62$&$5.50\pm0.22$&$-0.75\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-269&11:53:05.04&-18:18:36.6&$ 18.94$&$ 17.49$&$  7519.65$&$  6.7$&$  -6.9\pm       0.5$&$4747\pm  58$&$5.04\pm0.22$&$-0.72\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-270&11:52:39.79&-18:31:47.7&$ 18.95$&$ 17.46$&$  7519.65$&$  7.3$&$ -16.1\pm       0.6$&$4665\pm  80$&$5.35\pm0.29$&$-1.48\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-271&11:55:04.63&-18:43:41.1&$ 18.77$&$ 17.67$&$  7519.65$&$  1.7$&$  21.5\pm       0.7$&$4879\pm 133$&$5.16\pm0.36$&$ 1.08\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-272&11:54:19.71&-18:11:59.1&$ 18.88$&$ 17.51$&$  7519.65$&$  5.8$&$ 129.1\pm       0.6$&$4762\pm  78$&$4.49\pm0.28$&$-1.14\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-273&11:53:05.48&-18:40:00.3&$ 18.98$&$ 17.49$&$  7519.65$&$  5.3$&$ -13.3\pm       0.5$&$4605\pm  67$&$5.00\pm0.21$&$-0.02\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-274&11:52:01.90&-18:12:19.5&$ 19.00$&$ 17.38$&$  7519.65$&$  3.9$&$ -14.9\pm       0.7$&$4482\pm  64$&$5.24\pm0.28$&$-0.59\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-275&11:54:47.56&-18:35:10.1&$ 18.82$&$ 17.67$&$  7519.65$&$  2.7$&$  21.6\pm       0.5$&$4591\pm  86$&$4.44\pm0.25$&$ 0.24\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-276&11:53:21.20&-18:26:51.7&$ 19.05$&$ 17.58$&$  7519.65$&$  5.7$&$  21.9\pm       0.5$&$4765\pm  58$&$4.92\pm0.28$&$-0.22\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-277&11:54:54.25&-18:44:58.4&$ 19.10$&$ 17.66$&$  7519.65$&$  2.4$&$  61.2\pm       0.6$&$4920\pm  93$&$5.19\pm0.30$&$ 0.61\pm0.15$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-278&11:53:00.82&-18:15:03.0&$ 18.83$&$ 17.73$&$  7519.65$&$  6.0$&$  74.8\pm       0.4$&$4997\pm  52$&$4.84\pm0.17$&$ 0.18\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-279&11:53:06.65&-18:32:06.9&$ 18.85$&$ 17.70$&$  7519.65$&$  6.3$&$  59.7\pm       0.5$&$4981\pm  58$&$4.79\pm0.19$&$-0.34\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-280&11:54:35.11&-18:29:53.1&$ 18.89$&$ 17.65$&$  7519.65$&$  2.8$&$  28.2\pm       0.5$&$4631\pm  86$&$4.55\pm0.25$&$ 0.37\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-281&11:54:34.57&-18:44:23.9&$ 18.85$&$ 17.75$&$  7519.65$&$  0.4$&$  92.6\pm       1.2$&$4657\pm 175$&$4.64\pm0.55$&$ 0.42\pm0.30$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-282&11:52:31.88&-18:37:45.0&$ 19.15$&$ 17.51$&$  7519.65$&$  5.5$&$ -14.8\pm       0.9$&$4670\pm  91$&$5.60\pm0.22$&$-1.18\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-283&11:54:15.91&-18:03:57.5&$ 18.84$&$ 17.79$&$  7519.65$&$  0.8$&$  80.8\pm       1.4$&$4745\pm 259$&$3.74\pm0.87$&$ 0.79\pm0.41$\\%$0.000_{-0.000}^{+0.000}$
Cra2-284&11:52:48.52&-18:38:08.6&$ 19.11$&$ 17.69$&$  7519.65$&$  3.7$&$  12.8\pm       0.6$&$4515\pm  75$&$5.27\pm0.25$&$-0.25\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-285&11:53:39.40&-18:09:24.1&$ 18.92$&$ 17.77$&$  7519.65$&$  6.2$&$  81.5\pm       0.5$&$4815\pm  67$&$4.72\pm0.27$&$-0.62\pm0.10$\\%$0.000_{-0.000}^{+0.000}$
Cra2-286&11:54:15.70&-18:50:38.3&$ 18.89$&$ 17.82$&$  7519.65$&$  1.2$&$   5.9\pm       0.8$&$4915\pm 153$&$5.11\pm0.44$&$ 1.12\pm0.22$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-287&11:53:17.13&-18:03:28.3&$ 18.95$&$ 17.81$&$  7519.65$&$  6.7$&$  -0.7\pm       0.6$&$4904\pm  82$&$4.38\pm0.25$&$-1.27\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-288&11:53:45.78&-18:50:40.7&$ 19.16$&$ 17.72$&$  7519.65$&$  1.1$&$  18.1\pm       0.8$&$4550\pm 103$&$5.13\pm0.36$&$ 0.46\pm0.15$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-289&11:55:14.22&-18:26:28.0&$ 19.17$&$ 17.74$&$  7519.65$&$  4.0$&$  79.3\pm       0.6$&$4647\pm  88$&$4.35\pm0.28$&$-1.00\pm0.14$\\%$0.000_{-0.000}^{+0.001}$
Cra2-290&11:52:24.69&-18:23:22.0&$ 19.12$&$ 17.85$&$  7519.65$&$  5.5$&$  -0.1\pm       0.6$&$4683\pm  81$&$4.80\pm0.26$&$-0.77\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-291&11:52:22.21&-18:39:18.3&$ 19.13$&$ 17.89$&$  7519.65$&$  4.2$&$   4.4\pm       0.6$&$4861\pm  74$&$4.83\pm0.29$&$-0.15\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-292&11:52:25.48&-18:39:26.1&$ 19.28$&$ 17.81$&$  7519.65$&$  4.8$&$ -38.9\pm       1.0$&$4763\pm  98$&$5.44\pm0.29$&$-1.23\pm0.14$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-293&11:52:14.59&-18:35:08.4&$ 19.04$&$ 17.95$&$  7519.65$&$  6.2$&$  22.9\pm       0.6$&$5252\pm  83$&$5.43\pm0.25$&$-0.80\pm0.10$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-294&11:53:55.32&-18:10:45.6&$ 19.18$&$ 17.91$&$  7519.65$&$  4.8$&$   6.1\pm       0.7$&$5174\pm 111$&$5.05\pm0.37$&$-0.72\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-295&11:53:17.74&-18:09:22.5&$ 19.33$&$ 17.91$&$  7519.65$&$  6.8$&$  -2.1\pm       1.0$&$4872\pm 145$&$4.57\pm0.34$&$-1.94\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-296&11:52:34.39&-18:23:22.8&$ 19.27$&$ 17.93$&$  7519.65$&$  5.2$&$  31.3\pm       0.6$&$5000\pm  74$&$5.46\pm0.28$&$-0.66\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-297&11:54:57.70&-18:49:18.4&$ 19.04$&$ 18.04$&$  7519.65$&$  0.2$&$ -71.7\pm       1.3$&$4896\pm 232$&$4.72\pm0.75$&$ 1.00\pm0.32$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-298&11:54:55.31&-18:36:28.0&$ 19.12$&$ 18.03$&$  7519.65$&$  0.3$&$  79.6\pm       1.0$&$4663\pm 209$&$3.81\pm0.89$&$ 0.97\pm0.28$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-299&11:52:13.50&-18:27:49.1&$ 19.17$&$ 17.93$&$  7519.65$&$  5.9$&$  18.5\pm       0.9$&$5202\pm 145$&$4.88\pm0.34$&$-1.34\pm0.18$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-300&11:54:36.35&-18:30:53.0&$ 19.16$&$ 18.04$&$  7519.65$&$  2.5$&$  63.1\pm       0.7$&$4651\pm 117$&$4.73\pm0.33$&$-0.43\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-301&11:54:43.84&-18:31:54.3&$ 19.33$&$ 18.02$&$  7519.65$&$  0.6$&$   2.4\pm       1.0$&$4789\pm 191$&$5.06\pm0.57$&$ 1.05\pm0.27$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-302&11:52:25.57&-18:48:50.4&$ 19.17$&$ 18.09$&$  7519.65$&$  3.1$&$  13.8\pm       0.7$&$4835\pm 114$&$5.09\pm0.37$&$-0.45\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-303&11:55:04.21&-18:19:15.6&$ 19.40$&$ 18.04$&$  7519.65$&$  5.8$&$ -28.4\pm       1.5$&$4577\pm 108$&$4.97\pm0.40$&$-2.90\pm0.15$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-304&11:53:12.48&-18:26:20.0&$ 19.45$&$ 18.16$&$  7519.65$&$  5.0$&$   4.6\pm       0.7$&$4932\pm  86$&$4.67\pm0.27$&$-0.69\pm0.14$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-305&11:52:03.56&-18:42:31.8&$ 19.18$&$ 18.18$&$  7519.65$&$  3.1$&$ -10.3\pm       0.7$&$4876\pm 102$&$4.68\pm0.32$&$ 0.16\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-306&11:53:20.35&-18:33:17.8&$ 19.16$&$ 18.25$&$  7519.65$&$  1.5$&$ 123.0\pm       0.9$&$4649\pm 169$&$1.77\pm0.59$&$-0.46\pm0.26$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-307&11:52:05.34&-18:29:03.3&$ 19.29$&$ 18.13$&$  7519.65$&$  4.8$&$  19.1\pm       1.3$&$5043\pm 178$&$4.87\pm0.39$&$-1.65\pm0.23$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-308&11:53:21.97&-18:32:28.5&$ 19.33$&$ 18.22$&$  7519.65$&$  5.0$&$  44.9\pm       0.8$&$5023\pm 158$&$3.67\pm0.41$&$-1.49\pm0.23$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-309&11:53:58.04&-18:37:22.5&$ 19.31$&$ 18.16$&$  7519.65$&$  1.4$&$ 254.8\pm       1.2$&$4800\pm 171$&$4.91\pm0.54$&$-0.46\pm0.30$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-310&11:53:53.09&-18:26:31.2&$ 19.26$&$ 18.24$&$  7519.65$&$  8.1$&$ -27.9\pm       1.6$&$5127\pm 663$&$2.64\pm0.95$&$-2.91\pm0.71$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-311&11:54:11.60&-18:56:01.0&$ 19.41$&$ 18.19$&$  7519.65$&$  0.4$&$  24.0\pm       1.6$&$4899\pm 199$&$5.30\pm0.44$&$ 0.43\pm0.29$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-312&11:54:39.03&-18:43:45.5&$ 19.47$&$ 18.26$&$  7519.65$&$  1.5$&$   1.4\pm       0.9$&$4987\pm 123$&$5.19\pm0.38$&$ 0.48\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-313&11:52:07.08&-18:40:57.0&$ 19.38$&$ 18.24$&$  7519.65$&$  1.8$&$ 102.3\pm       0.9$&$4466\pm  60$&$4.35\pm0.37$&$-0.11\pm0.16$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-314&11:51:45.95&-18:19:45.7&$ 19.29$&$ 18.32$&$  7519.65$&$  5.2$&$   4.1\pm       1.4$&$5021\pm 312$&$4.49\pm0.46$&$-2.17\pm0.37$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-315&11:53:22.64&-18:37:11.9&$ 19.31$&$ 18.27$&$  7519.65$&$  0.5$&$  -1.0\pm       1.0$&$4618\pm 163$&$3.42\pm0.61$&$ 0.74\pm0.26$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-316&11:53:21.54&-18:31:24.0&$ 19.27$&$ 18.31$&$  7519.65$&$  5.3$&$  70.3\pm       0.7$&$4858\pm 105$&$3.99\pm0.29$&$-1.37\pm0.15$\\%$0.000_{-0.000}^{+0.000}$
Cra2-317&11:54:14.92&-18:15:39.2&$ 19.42$&$ 18.36$&$  7519.65$&$  7.8$&$  -9.7\pm       1.4$&$5993\pm 784$&$3.92\pm0.88$&$-2.10\pm0.73$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-318&11:52:57.09&-18:25:45.4&$ 19.45$&$ 18.29$&$  7519.65$&$  3.9$&$ -12.8\pm       0.8$&$4603\pm 109$&$4.55\pm0.32$&$-1.06\pm0.13$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-319&11:54:20.53&-18:10:26.3&$ 19.54$&$ 18.26$&$  7519.65$&$  3.9$&$ 148.4\pm       0.9$&$5051\pm 108$&$5.52\pm0.28$&$-1.15\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-320&11:54:35.05&-18:41:36.6&$ 19.53$&$ 18.30$&$  7519.65$&$  1.5$&$  72.7\pm       0.9$&$4766\pm 119$&$4.96\pm0.48$&$ 0.13\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-321&11:52:13.68&-18:20:47.9&$ 19.43$&$ 18.31$&$  7519.65$&$  4.6$&$ 123.0\pm       0.8$&$4955\pm 149$&$4.97\pm0.42$&$-1.52\pm0.18$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-322&11:54:05.93&-18:06:29.7&$ 19.50$&$ 18.38$&$  7519.65$&$  2.8$&$  38.9\pm       0.7$&$4989\pm 101$&$4.16\pm0.33$&$-0.09\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-323&11:53:46.65&-18:25:04.7&$ 19.41$&$ 18.39$&$  7519.65$&$  4.7$&$  34.2\pm       1.0$&$5216\pm 156$&$4.97\pm0.42$&$-1.26\pm0.19$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-324&11:52:04.40&-18:40:04.3&$ 19.59$&$ 18.38$&$  7519.65$&$  5.5$&$ 157.5\pm       0.9$&$5002\pm 140$&$4.99\pm0.36$&$-1.61\pm0.19$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-325&11:52:33.62&-18:50:47.8&$ 19.45$&$ 18.39$&$  7519.65$&$  1.6$&$ 127.7\pm       1.3$&$4603\pm 148$&$4.66\pm0.63$&$-0.60\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-326&11:53:21.95&-18:49:45.5&$ 19.39$&$ 18.42$&$  7519.65$&$  0.8$&$ 113.3\pm       1.0$&$4861\pm 198$&$4.78\pm0.57$&$ 0.43\pm0.28$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-327&11:52:41.06&-18:24:08.8&$ 19.43$&$ 18.45$&$  7519.65$&$  3.8$&$  80.6\pm       0.8$&$4860\pm 146$&$4.82\pm0.39$&$-1.21\pm0.18$\\%$0.002_{-0.002}^{+0.010}$
Cra2-328&11:53:00.54&-18:13:34.3&$ 19.47$&$ 18.52$&$  7519.65$&$  7.3$&$  77.5\pm       1.5$&$4615\pm 122$&$4.61\pm0.34$&$-2.86\pm0.15$\\%$0.000_{-0.000}^{+0.002}$
Cra2-329&11:54:53.82&-18:14:07.2&$ 19.40$&$ 18.52$&$  7519.65$&$  3.8$&$  19.8\pm       1.0$&$5897\pm 343$&$4.97\pm0.49$&$-0.64\pm0.36$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-330&11:54:54.05&-18:28:24.4&$ 19.51$&$ 18.50$&$  7519.65$&$  1.0$&$  17.8\pm       0.8$&$5156\pm 167$&$5.15\pm0.43$&$ 1.01\pm0.26$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-331&11:53:11.67&-18:29:00.8&$ 19.62$&$ 18.52$&$  7519.65$&$  4.7$&$  41.5\pm       1.2$&$4615\pm 130$&$5.17\pm0.37$&$-2.46\pm0.17$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-332&11:55:13.28&-18:17:54.5&$ 18.11$&$ 16.57$&$  7519.65$&$  8.6$&$  -1.8\pm       0.3$&$4689\pm  35$&$4.72\pm0.13$&$ 0.09\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-333&11:52:34.28&-18:16:41.0&$ 19.53$&$ 18.61$&$  7519.65$&$  4.6$&$  86.8\pm       1.0$&$4698\pm 155$&$3.79\pm0.36$&$-2.03\pm0.20$\\%$0.971_{-0.011}^{+0.006}$
Cra2-334&11:52:14.19&-18:23:22.1&$ 19.62$&$ 18.50$&$  7519.65$&$  3.9$&$  78.6\pm       0.8$&$4673\pm 128$&$3.58\pm0.36$&$-1.22\pm0.18$\\%$0.009_{-0.007}^{+0.039}$
Cra2-335&11:53:51.40&-18:20:25.8&$ 19.65$&$ 18.57$&$  7519.65$&$  2.6$&$  34.9\pm       0.9$&$5150\pm 115$&$4.96\pm0.39$&$-0.30\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-336&11:54:50.73&-18:21:07.8&$ 19.75$&$ 18.57$&$  7519.65$&$  1.4$&$ -36.2\pm       1.0$&$4884\pm 143$&$5.22\pm0.41$&$-0.31\pm0.20$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-337&11:52:26.09&-18:47:42.2&$ 19.62$&$ 18.61$&$  7519.65$&$  3.7$&$  74.9\pm       1.3$&$4928\pm 182$&$5.32\pm0.39$&$-1.73\pm0.24$\\%$0.000_{-0.000}^{+0.001}$
Cra2-338&11:52:52.07&-18:05:10.9&$ 19.79$&$ 18.66$&$  7519.65$&$  2.8$&$  80.8\pm       1.0$&$4513\pm  90$&$3.95\pm0.48$&$-1.11\pm0.16$\\%$0.004_{-0.004}^{+0.033}$
Cra2-339&11:52:30.61&-18:27:26.8&$ 19.64$&$ 18.70$&$  7519.65$&$  5.2$&$  98.3\pm       1.4$&$4806\pm 187$&$4.44\pm0.44$&$-2.17\pm0.25$\\%$0.013_{-0.011}^{+0.052}$
Cra2-340&11:54:16.62&-18:21:19.3&$ 19.70$&$ 18.70$&$  7519.65$&$  1.5$&$  92.5\pm       1.0$&$5037\pm 170$&$5.36\pm0.44$&$-0.63\pm0.26$\\%$0.000_{-0.000}^{+0.000}$
Cra2-341&11:51:33.19&-18:41:17.8&$ 19.85$&$ 18.75$&$  7519.65$&$  2.9$&$  58.0\pm       1.2$&$4655\pm 151$&$3.50\pm0.39$&$-1.54\pm0.23$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-342&11:51:56.85&-18:19:41.1&$ 18.05$&$ 16.67$&$  7519.65$&$ 10.2$&$ -18.0\pm       0.3$&$4769\pm  36$&$4.93\pm0.14$&$ 0.00\pm0.05$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-343&11:54:45.21&-18:37:18.6&$ 19.72$&$ 18.82$&$  7519.65$&$  4.7$&$ 127.8\pm       2.4$&$6296\pm 668$&$4.09\pm0.74$&$-1.48\pm0.56$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-344&11:53:05.30&-18:43:17.1&$ 19.73$&$ 18.78$&$  7519.65$&$  1.7$&$ 127.4\pm       1.9$&$4656\pm 187$&$4.66\pm0.61$&$-1.42\pm0.22$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-345&11:51:16.84&-18:28:50.2&$ 19.94$&$ 18.67$&$  7519.65$&$  1.4$&$  55.1\pm       1.4$&$4648\pm 182$&$4.20\pm0.62$&$-0.99\pm0.29$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-346&11:53:39.31&-18:04:18.3&$ 18.07$&$ 16.67$&$  7519.65$&$ 11.6$&$  24.5\pm       0.4$&$4895\pm  41$&$4.87\pm0.16$&$-0.38\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-347&11:52:39.69&-18:10:14.2&$ 19.96$&$ 18.76$&$  7519.65$&$  4.8$&$  93.6\pm       1.3$&$4541\pm 103$&$4.78\pm0.45$&$-2.58\pm0.19$\\%$0.045_{-0.037}^{+0.157}$
Cra2-348&11:52:24.61&-18:30:11.2&$ 19.75$&$ 18.83$&$  7519.65$&$  3.0$&$ 174.5\pm       1.3$&$5067\pm 220$&$4.87\pm0.52$&$-1.48\pm0.27$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-349&11:52:44.19&-18:40:51.9&$ 19.86$&$ 18.88$&$  7519.65$&$  3.4$&$  68.7\pm       1.2$&$5846\pm 261$&$5.38\pm0.36$&$-0.59\pm0.29$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-350&11:52:36.58&-18:42:22.1&$ 19.83$&$ 18.86$&$  7519.65$&$  1.9$&$ 162.7\pm       1.7$&$4918\pm 278$&$4.89\pm0.56$&$-1.41\pm0.32$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-351&11:53:32.26&-18:28:36.9&$ 19.87$&$ 18.90$&$  7519.65$&$  3.7$&$  29.4\pm       1.4$&$6161\pm 313$&$5.31\pm0.43$&$-0.73\pm0.30$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-352&11:52:16.94&-18:55:03.0&$ 19.86$&$ 18.94$&$  7519.65$&$  1.8$&$  -7.2\pm       1.3$&$5371\pm 215$&$5.37\pm0.40$&$-0.19\pm0.27$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-353&11:53:13.37&-18:34:50.0&$ 19.77$&$ 19.01$&$  7519.65$&$  2.0$&$ 306.0\pm       1.9$&$5232\pm 220$&$5.55\pm0.31$&$-1.38\pm0.28$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-354&11:53:11.75&-18:07:33.0&$ 19.83$&$ 18.98$&$  7519.65$&$  3.5$&$ 112.2\pm       2.5$&$4804\pm 327$&$4.23\pm0.83$&$-2.91\pm0.36$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-355&11:53:00.68&-18:49:53.3&$ 18.22$&$ 16.59$&$  7519.65$&$  6.5$&$  31.5\pm       0.4$&$4433\pm  31$&$5.10\pm0.13$&$ 0.21\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-356&11:53:32.73&-18:36:39.7&$ 18.15$&$ 16.70$&$  7519.65$&$  5.3$&$  28.7\pm       0.7$&$4505\pm  81$&$4.80\pm0.27$&$ 0.66\pm0.12$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-357&11:54:07.25&-18:04:26.3&$ 20.20$&$ 19.13$&$  7519.65$&$  1.6$&$ 169.0\pm       3.0$&$5549\pm 608$&$4.93\pm0.71$&$-1.69\pm0.68$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-358&11:52:41.80&-18:09:43.4&$ 20.08$&$ 19.35$&$  7519.65$&$  3.6$&$  91.0\pm       3.2$&$4667\pm 226$&$4.57\pm0.77$&$-2.89\pm0.36$\\%$0.248_{-0.142}^{+0.210}$
Cra2-359&11:53:58.21&-18:13:59.8&$ 20.37$&$ 19.40$&$  7519.65$&$  2.5$&$ 176.6\pm       2.0$&$5339\pm 491$&$4.11\pm0.87$&$-1.85\pm0.52$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-360&11:53:14.42&-18:30:52.7&$ 20.35$&$ 19.40$&$  7519.65$&$  2.0$&$ 223.8\pm       2.7$&$5887\pm 436$&$5.38\pm0.42$&$-1.07\pm0.56$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-361&11:54:37.14&-18:53:25.4&$ 18.23$&$ 16.82$&$  7519.65$&$  4.1$&$  42.4\pm       0.4$&$4606\pm  71$&$5.01\pm0.20$&$ 0.69\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-362&11:52:24.70&-18:05:23.2&$ 18.54$&$ 16.79$&$  7519.65$&$  7.7$&$  40.0\pm       0.5$&$4544\pm  70$&$4.95\pm0.23$&$-1.01\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-363&11:54:21.66&-18:26:07.5&$ 18.35$&$ 16.93$&$  7519.65$&$  8.1$&$  27.3\pm       0.4$&$4834\pm  40$&$4.70\pm0.15$&$-0.23\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-364&11:54:37.78&-18:20:25.5&$ 18.60$&$ 16.83$&$  7519.65$&$  7.4$&$  29.7\pm       0.5$&$4796\pm  63$&$4.76\pm0.29$&$-0.94\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-365&11:54:49.15&-18:28:12.0&$ 18.48$&$ 16.88$&$  7519.65$&$  8.5$&$  34.4\pm       0.5$&$4855\pm  56$&$4.69\pm0.21$&$-0.88\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-366&11:54:41.48&-18:17:07.2&$ 18.56$&$ 16.90$&$  7519.65$&$  7.7$&$  68.5\pm       0.4$&$4739\pm  52$&$4.87\pm0.28$&$-0.67\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-367&11:54:50.20&-18:25:07.4&$ 18.45$&$ 17.01$&$  7519.65$&$  8.2$&$  36.1\pm       0.4$&$5002\pm  43$&$5.07\pm0.17$&$-0.09\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-368&11:53:15.82&-18:23:06.3&$ 18.41$&$ 16.97$&$  7519.65$&$  9.1$&$  22.7\pm       0.4$&$4806\pm  46$&$5.28\pm0.18$&$-0.48\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-369&11:54:26.48&-18:38:58.1&$ 18.51$&$ 17.01$&$  7519.65$&$  5.1$&$  14.3\pm       0.5$&$4803\pm  55$&$5.56\pm0.21$&$-0.30\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-370&11:55:08.86&-18:30:37.2&$ 18.37$&$ 17.11$&$  7519.65$&$  6.2$&$  33.9\pm       0.4$&$4971\pm  42$&$5.26\pm0.13$&$ 0.53\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-371&11:53:04.63&-18:22:49.2&$ 18.33$&$ 17.14$&$  7519.65$&$  9.8$&$  38.0\pm       0.4$&$4912\pm  43$&$4.88\pm0.15$&$-0.55\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-372&11:52:31.66&-18:39:30.6&$ 18.51$&$ 17.09$&$  7519.65$&$  6.4$&$  21.4\pm       0.4$&$4688\pm  48$&$5.16\pm0.15$&$ 0.07\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-373&11:53:20.03&-18:39:12.5&$ 18.40$&$ 17.14$&$  7519.65$&$  6.1$&$  24.0\pm       0.4$&$4661\pm  59$&$5.07\pm0.18$&$ 0.34\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-374&11:52:22.35&-18:48:06.6&$ 18.61$&$ 17.15$&$  7519.65$&$  4.9$&$   3.8\pm       0.4$&$4770\pm  59$&$5.07\pm0.18$&$ 0.44\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-375&11:53:31.99&-18:07:00.9&$ 18.40$&$ 17.19$&$  7519.65$&$ 10.7$&$ 166.6\pm       0.6$&$4728\pm  79$&$4.34\pm0.21$&$-2.03\pm0.11$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-376&11:54:58.74&-18:32:19.4&$ 18.49$&$ 17.26$&$  7519.65$&$  5.1$&$  12.7\pm       0.4$&$4933\pm  49$&$5.43\pm0.17$&$ 0.18\pm0.06$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-377&11:52:49.92&-18:22:53.2&$ 18.60$&$ 17.20$&$  7519.65$&$  8.0$&$  29.8\pm       0.4$&$4825\pm  54$&$5.18\pm0.24$&$-0.60\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-378&11:54:37.32&-18:15:31.8&$ 18.69$&$ 17.19$&$  7519.65$&$  6.0$&$ 112.8\pm       0.5$&$4805\pm  46$&$4.80\pm0.18$&$ 0.00\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-379&11:53:12.43&-18:20:20.7&$ 18.72$&$ 17.14$&$  7519.65$&$  8.3$&$ 145.7\pm       0.5$&$4665\pm  59$&$4.92\pm0.24$&$-1.07\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-380&11:52:44.91&-18:33:44.9&$ 18.57$&$ 17.22$&$  7519.65$&$  7.8$&$ 197.8\pm       0.6$&$4544\pm  90$&$5.16\pm0.21$&$-2.13\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-381&11:52:13.22&-18:51:47.8&$ 18.72$&$ 17.22$&$  7519.65$&$  6.4$&$  31.8\pm       0.5$&$4482\pm  58$&$5.26\pm0.22$&$-0.82\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-382&11:52:54.52&-18:16:19.2&$ 18.78$&$ 17.18$&$  7519.65$&$  8.3$&$  21.9\pm       0.6$&$4498\pm  65$&$4.90\pm0.23$&$-1.53\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-383&11:54:42.22&-18:30:14.7&$ 18.58$&$ 17.33$&$  7519.65$&$  5.9$&$  14.2\pm       0.4$&$5168\pm  44$&$5.64\pm0.16$&$-0.01\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-384&11:51:32.03&-18:31:03.2&$ 18.83$&$ 17.24$&$  7519.65$&$  3.8$&$  25.7\pm       0.5$&$4428\pm  29$&$5.25\pm0.20$&$-0.13\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-385&11:52:34.94&-18:34:08.8&$ 18.51$&$ 17.37$&$  7519.65$&$  7.3$&$  -2.7\pm       0.4$&$4913\pm  53$&$5.03\pm0.18$&$-0.56\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-386&11:54:03.81&-18:32:31.3&$ 18.82$&$ 17.23$&$  7519.65$&$  2.9$&$ -30.2\pm       0.5$&$4503\pm  69$&$5.01\pm0.21$&$ 0.52\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-387&11:51:31.81&-18:42:26.0&$ 18.64$&$ 17.46$&$  7519.65$&$  6.1$&$   2.3\pm       0.5$&$4955\pm  50$&$4.98\pm0.16$&$ 0.15\pm0.07$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-388&11:54:01.66&-18:24:33.6&$ 18.63$&$ 17.41$&$  7519.65$&$  5.6$&$  83.2\pm       0.4$&$4948\pm  55$&$5.02\pm0.22$&$-0.22\pm0.08$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-389&11:54:25.30&-18:06:21.0&$ 18.95$&$ 17.34$&$  7519.65$&$  5.3$&$  14.5\pm       0.5$&$4861\pm  60$&$5.22\pm0.28$&$-0.31\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
Cra2-390&11:52:35.99&-18:22:20.1&$ 18.86$&$ 17.44$&$  7519.65$&$  7.4$&$ -24.0\pm       0.5$&$5016\pm  57$&$5.49\pm0.21$&$-0.60\pm0.09$\\%$0.000_{ 0.000}^{+0.000}$
\hline
\end{tabular}
\\
\raggedright
$^{a}$median signal-to-noise ratio per pixel\\
$^{b}$ heliocentric Julian date minus $2.45\times 10^6$ days\\
$^{c}$median signal-to-noise ratio per pixel\\
$^{d}$line-of-sight velocity in the heliocentric rest frame\\
\label{tab:cra2_table1}
\end{table*}

